Robust Invisible Video Watermarking with Attention

The goal of video watermarking is to embed a message within a video file in a way such that it minimally impacts the viewing experience but can be recovered even if the video is redistributed and modified, allowing media producers to assert ownership over their content. This paper presents RivaGAN, a novel architecture for robust video watermarking which features a custom attention-based mechanism for embedding arbitrary data as well as two independent adversarial networks which critique the video quality and optimize for robustness. Using this technique, we are able to achieve state-of-the-art results in deep learning-based video watermarking and produce watermarked videos which have minimal visual distortion and are robust against common video processing operations.

==> misc.tex <==

%----- Coarse, broad, general definition
%Video watermarking can be broadly defined as the set of techniques that aim at hiding additional information, namely a \textit{bit vector}, into a video sequence while preserving the quality and fidelity of the image. 
%Additionally, it is usually desirable the watermark to be hard to remove or modify. %\cite{GuidedTourOfVideoWatermarking}.

%----- Applications, listed according to the agents involved in a video transmission
%Video watermarking is applicable to all the different agents involved in a video sequence cycle of life, whatever its purpose or lifespan is \cite{OverviewOfDigitalWatermarking}. 
%
%Thus, the owner or creator can prove ownership of the content, even after it has been distributed, by embedding copyright information.
%
%Producers can help video sharing websites to detect copyright infringement and copy control more accurately than existing video fingerprinting techniques by embedding identifiers,
%
%Likewise, distributors can identify leakers by extracting the unique identifier from the leaked content.
%
%Embedding tags related to the content and rating helps audience to search-and-find, and parents to filter out.
%
%Finally, makes possible for advertisers to be sure that the time slots acquired are indeed used to air their commercials by automated broadcast monitoring.
